Measurement of sin^2\theta_{eff}^{lept} and Z-light quark couplings using the forward-backward charge asymmetry in p\bar{p} -> Z/\gamma^{*} -> e^{+}e^{-} events with L=5.0 fb^{-1} at \sqrt{s}=1.96 TeV

We measure the mass dependence of the forward-backward charge asymmetry in 157,553 $p\bar{p} \rightarrow Z/\gamma^{*} \rightarrow e^+e^-$ interactions, corresponding to 5.0 fb$^{-1}$ of integrated luminosity collected by the D0 experiment at the Fermilab Tevatron Collider at $\sqrt{s}=1.96$ TeV. The effective weak mixing angle ($\sin^2\theta_{eff}^{lept}$) from this process involving predominantly the first generation of quarks is extracted as $\sin^2\theta_{eff}^{lept} = 0.2309 \pm 0.0008 ({stat.}) \pm 0.0006 ({syst.})$. We also present the most precise direct measurement of the vector and axial-vector couplings of $u$ and $d$ quarks to the $Z$ boson.

==> compare.tex <==
\begin{figure}[htbp]
\epsfig{file=figures/DZero_AFB_ee_InvMass_All.eps,scale=0.45}
\caption{\small Comparisons of the dielectron invariant mass between data and the sum of 
signal and background predictions for combined CC and CE events. 
The insert focuses on the $Z$ pole region from 50~GeV 
to 130~GeV, where good agreement between data and the sum of signal and 
background predictions is essential to perform the unfolding.}
\label{fig5:invmass}
\end{figure}

\begin{figure}[htbp]
\epsfig{file=figures/DZero_AFB_ee_Collin_All.eps,scale=0.45}
\caption{\small Comparisons of the $\cos \theta^{*}$ between data and the sum of signal and background predictions for combined CC and CE events.} 
\label{fig5:collin}
\end{figure}


==> data_num.tex <==
{\begingroup
\begin{table*}
\begin{center}
\caption{Numbers of forward and backward CC and CE events 
in each $M_{ee}$ bin after all selections.}
\begin{tabular}{r@{$\, - \,$}lcccc}
\hline
\hline
\multicolumn{2}{c}{\multirow{2}{*}{$M_{ee}$ (GeV)}}  & \multicolumn{2}{c}{ CC}  &  \multicolumn{2}{c}{ CE} \\ %\cline{2-5}
               \multicolumn{2}{c}{}  & Forward & Backward & Forward & Backward \\ \cline{1-6}
50 & 60 & 276 & 319 & 54 & 70 \\ 
60 & 70 & 464 & 711 & 238 & 413 \\ 
70 & 75 & 411 & 545 & 285 & 495 \\ 
75 & 81 & 852 & 1062 & 778 & 1240 \\ 
81 & 86.5 & 3359 & 3559 & 3804 & 4245 \\
86.5 & 89.5 & 6681 & 6642 & 8339 & 7591 \\ 
89.5 & 92 & 9297 & 8717 & 11098 & 9534 \\ 
92 & 97 & 12076 & 11109 & 14281 & 11412 \\ 
97 & 105 & 2890 & 2173 & 3711 & 2150 \\ 
105 & 115 & 680 & 431 & 1125 & 395 \\ 
115 & 130 & 408 & 189 & 764 & 229 \\ 
130 & 180 & 439 & 150 & 845 & 269 \\ 
180 & 250 & 138 & 61 & 229 & 73 \\ 
250 & 500 & 63 & 45 & 86 & 24 \\ 
500 & 1000 & 7 & 1 & 1 & 0 \\ \hline 
\hline
\end{tabular}
\label{Tab:data_num}
\end{center}
\end{table*}
\endgroup}

